Effective computation of centralizers of ODOs

This work is devoted to computing the centralizer $Z (L)$ of an ordinary differential operator (ODO) in the ring of differential operators. Non-trivial centralizers are known to be coordinate rings of spectral curves and contain the ring of polynomials $C [L]$, with coefficients in the field of constants $C$ of $L$. We give an algorithm to compute a basis of $Z (L)$ as a $C [L]$-module. Our approach combines results by K. Goodearl in 1985 with solving the systems of equations of the stationary Gelfand-Dickey (GD) hierarchy, which after substituting the coefficients of $L$ become linear, and whose solution sets form a flag of constants. We are assuming that the coefficients of $L$ belong to a differential algebraic extension $K$ of $C$. In addition, by considering parametric coefficients we develop an algorithm to generate families of ODOs with non trivial centralizer, in particular algebro-geometric, whose coefficients are solutions in $K$ of systems of the stationary GD hierarchy.

==> table1.tex <==
\begin{table}[!ht]
\centering \tiny
\caption{Execution time (in seconds) for computing the order $m$ almost commuting basis element for the operator $L_n$ using different approaches.}
\label{tab:comparison}
\begin{adjustbox}{center}
\begin{tabular}{cc|rrrr|rr|rr|r}
\toprule
 &  & \textbf{D.I.} & \textbf{D.L.} & \textbf{R.I.} & \textbf{R.L.} & \textbf{D.I./D.L.} & \textbf{D.I./R.I.} & \textbf{D.L./R.L.} & \textbf{R.I./R.L.} & \textbf{D.I./R.L.} \\
n & m &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[t]{4}{*}{2} & 3 & 2.106003 & 0.617583 & 1.001537 & \bfseries 0.273354 & 3.410071 & 2.102771 & 2.259279 & 3.663881 & 7.704302 \\
 & 5 & 21.011702 & 1.836433 & 11.514676 & \bfseries 1.016280 & 11.441587 & 1.824776 & 1.807014 & 11.330220 & 20.675112 \\
 & 7 & 152.211611 & 5.472876 & 90.705532 & \bfseries 3.983174 & 27.811997 & 1.678085 & 1.373999 & 22.772175 & 38.213649 \\
 & 9 & 839.699525 & 18.758223 & 542.146459 & \bfseries 16.089755 & 44.764342 & 1.548843 & 1.165849 & 33.695134 & 52.188458 \\
\midrule
\multirow[t]{6}{*}{3} & 2 & 1.292478 & 0.531627 & 0.639675 & \bfseries 0.196769 & 2.431172 & 2.020522 & 2.701789 & 3.250900 & 6.568515 \\
 & 4 & 14.488225 & 1.890632 & 5.499801 & \bfseries 0.942575 & 7.663167 & 2.634318 & 2.005816 & 5.834870 & 15.370902 \\
 & 5 & 41.510969 & 3.482110 & 17.715803 & \bfseries 2.093283 & 11.921213 & 2.343160 & 1.663468 & 8.463167 & 19.830557 \\
 & 7 & 223.432386 & 15.980079 & 106.905031 & \bfseries 13.216854 & 13.981933 & 2.090008 & 1.209068 & 8.088538 & 16.905111 \\
 & 8 & 544.310636 & 37.609066 & 259.083967 & \bfseries 33.799681 & 14.472857 & 2.100904 & 1.112705 & 7.665278 & 16.104017 \\
 & 10 & 2470.133394 & 214.397025 & 1427.103806 & \bfseries 206.493211 & 11.521304 & 1.730872 & 1.038276 & 6.911142 & 11.962298 \\
\midrule
\multirow[t]{7}{*}{4} & 2 & 2.454977 & 0.766286 & 1.243150 & \bfseries 0.246464 & 3.203733 & 1.974804 & 3.109122 & 5.043942 & 9.960798 \\
 & 3 & 8.913038 & 1.387575 & 3.392211 & \bfseries 0.512681 & 6.423466 & 2.627501 & 2.706505 & 6.616607 & 17.385142 \\
 & 5 & 62.335976 & 5.044560 & 20.345616 & \bfseries 2.963571 & 12.357069 & 3.063853 & 1.702189 & 6.865236 & 21.034073 \\
 & 6 & 153.221437 & 11.271272 & 54.621827 & \bfseries 8.201267 & 13.593979 & 2.805132 & 1.374333 & 6.660169 & 18.682654 \\
 & 7 & 352.584263 & 26.075651 & 134.789081 & \bfseries 22.369181 & 13.521590 & 2.615822 & 1.165695 & 6.025660 & 15.762055 \\
 & 9 & 1687.035697 & 183.774950 & 740.973020 & \bfseries 173.549791 & 9.179900 & 2.276784 & 1.058918 & 4.269513 & 9.720759 \\
 & 10 & 3063.436515 & \bfseries 486.916002 & 1252.616465 & nan & 6.291509 & 2.445630 & nan & nan & nan \\
\midrule
\multirow[t]{7}{*}{5} & 2 & 4.456064 & 1.067041 & 2.343569 & \bfseries 0.310524 & 4.176093 & 1.901400 & 3.436258 & 7.547139 & 14.350133 \\
 & 3 & 14.967405 & 1.938808 & 6.312084 & \bfseries 0.646967 & 7.719901 & 2.371230 & 2.996765 & 9.756422 & 23.134725 \\
 & 4 & 39.805168 & 3.433828 & 12.869442 & \bfseries 1.471362 & 11.592069 & 3.092999 & 2.333775 & 8.746618 & 27.053278 \\
 & 6 & 217.317041 & 14.358385 & 63.055707 & \bfseries 10.082573 & 15.135201 & 3.446429 & 1.424079 & 6.253930 & 21.553728 \\
 & 7 & 509.996037 & 34.038148 & 158.828582 & \bfseries 28.008855 & 14.983072 & 3.210984 & 1.215264 & 5.670656 & 18.208386 \\
 & 8 & 1088.602051 & 92.102915 & 368.830461 & \bfseries 81.915048 & 11.819409 & 2.951497 & 1.124371 & 4.502597 & 13.289403 \\
 & 9 & 2062.130642 & 254.742405 & 802.165949 & \bfseries 238.970028 & 8.094964 & 2.570703 & 1.066001 & 3.356764 & 8.629244 \\
\midrule
\multirow[t]{8}{*}{6} & 2 & 7.449102 & 1.476193 & 4.230699 & \bfseries 0.402960 & 5.046156 & 1.760726 & 3.663375 & 10.499056 & 18.485960 \\
 & 3 & 24.571622 & 2.592874 & 10.838114 & \bfseries 0.817929 & 9.476597 & 2.267149 & 3.170049 & 13.250682 & 30.041275 \\
 & 4 & 59.909523 & 4.374745 & 21.405684 & \bfseries 1.810230 & 13.694404 & 2.798767 & 2.416679 & 11.824842 & 33.094979 \\
 & 5 & 140.293024 & 7.928903 & 39.919621 & \bfseries 4.133238 & 17.693876 & 3.514388 & 1.918327 & 9.658195 & 33.942642 \\
 & 7 & 688.762805 & 40.384600 & 178.744432 & \bfseries 31.765289 & 17.055085 & 3.853339 & 1.271344 & 5.627036 & 21.682875 \\
 & 8 & 1494.395439 & 107.559769 & 423.402639 & \bfseries 94.410162 & 13.893628 & 3.529490 & 1.139282 & 4.484715 & 15.828756 \\
 & 9 & 2707.648989 & 299.880491 & 893.060088 & \bfseries 283.335145 & 9.029093 & 3.031878 & 1.058395 & 3.151957 & 9.556347 \\
 & 10 & 5135.524964 & \bfseries 896.025691 & 1940.418949 & nan & 5.731448 & 2.646606 & nan & nan & nan \\
\midrule
\multirow[t]{8}{*}{7} & 2 & 12.259338 & 1.899759 & 7.239116 & \bfseries 0.508820 & 6.453103 & 1.693486 & 3.733655 & 14.227259 & 24.093658 \\
 & 3 & 38.434121 & 3.252893 & 18.067635 & \bfseries 1.007010 & 11.815366 & 2.127236 & 3.230250 & 17.941869 & 38.166588 \\
 & 4 & 91.256922 & 5.473903 & 34.818924 & \bfseries 2.140145 & 16.671271 & 2.620900 & 2.557725 & 16.269424 & 42.640534 \\
 & 5 & 206.836224 & 9.498544 & 65.076246 & \bfseries 4.752244 & 21.775571 & 3.178367 & 1.998749 & 13.693793 & 43.523906 \\
 & 6 & 438.436775 & 19.813827 & 112.686891 & \bfseries 12.637371 & 22.127819 & 3.890752 & 1.567876 & 8.916957 & 34.693670 \\
 & 8 & 1906.229007 & 118.513882 & 472.455922 & \bfseries 103.099357 & 16.084437 & 4.034723 & 1.149511 & 4.582530 & 18.489243 \\
 & 9 & 3898.616881 & 331.131072 & 903.611645 & \bfseries 305.686101 & 11.773637 & 4.314483 & 1.083239 & 2.956012 & 12.753661 \\
 & 10 & 6945.082992 & \bfseries 1007.526896 & 2234.549951 & nan & 6.893199 & 3.108046 & nan & nan & nan \\
\midrule
\multirow[t]{8}{*}{8} & 2 & 19.546785 & 2.471947 & 12.028045 & \bfseries 0.648746 & 7.907445 & 1.625101 & 3.810344 & 18.540441 & 30.130085 \\
 & 3 & 57.931595 & 4.143153 & 29.175311 & \bfseries 1.273873 & 13.982490 & 1.985638 & 3.252406 & 22.902836 & 45.476733 \\
 & 4 & 132.788908 & 6.711907 & 54.697211 & \bfseries 2.563208 & 19.784081 & 2.427709 & 2.618557 & 21.339359 & 51.805752 \\
 & 5 & 286.300140 & 11.597983 & 97.180613 & \bfseries 5.566635 & 24.685339 & 2.946062 & 2.083482 & 17.457694 & 51.431454 \\
 & 6 & 580.526930 & 22.108047 & 151.583063 & \bfseries 14.012471 & 26.258626 & 3.829761 & 1.577741 & 10.817726 & 41.429305 \\
 & 7 & 1241.237437 & 49.338820 & 303.007566 & \bfseries 37.011899 & 25.157421 & 4.096391 & 1.333053 & 8.186761 & 33.536172 \\
 & 9 & 4822.763817 & 350.764575 & 1156.488116 & \bfseries 317.999015 & 13.749290 & 4.170180 & 1.103037 & 3.636766 & 15.165971 \\
 & 10 & nan & \bfseries 1058.891042 & 2334.787880 & nan & nan & nan & nan & nan & nan \\
\midrule
\multirow[t]{8}{*}{9} & 2 & 29.832844 & 3.095817 & 19.237077 & \bfseries 0.820667 & 9.636502 & 1.550799 & 3.772317 & 23.440780 & 36.351943 \\
 & 3 & 86.629985 & 5.056829 & 44.781074 & \bfseries 1.505004 & 17.131287 & 1.934522 & 3.360011 & 29.754797 & 57.561317 \\
 & 4 & 192.587451 & 8.299221 & 82.881520 & \bfseries 3.019709 & 23.205484 & 2.323648 & 2.748351 & 27.446857 & 63.776825 \\
 & 5 & 406.375658 & 13.725177 & 147.371403 & \bfseries 6.300055 & 29.608044 & 2.757493 & 2.178581 & 23.392083 & 64.503513 \\
 & 6 & 817.943497 & 25.176297 & 256.564884 & \bfseries 15.337580 & 32.488634 & 3.188057 & 1.641478 & 16.727860 & 53.329372 \\
 & 7 & 1689.210331 & 54.250515 & 439.815275 & \bfseries 39.452931 & 31.137222 & 3.840727 & 1.375069 & 11.147848 & 42.815839 \\
 & 8 & 3088.345060 & 137.680890 & 745.084940 & \bfseries 113.737114 & 22.431182 & 4.144957 & 1.210519 & 6.550939 & 27.153362 \\
 & 10 & nan & \bfseries 1110.683134 & 2478.840138 & nan & nan & nan & nan & nan & nan \\
\midrule
\multirow[t]{8}{*}{10} & 2 & 44.808236 & 3.840817 & 29.342092 & \bfseries 1.053197 & 11.666331 & 1.527098 & 3.646817 & 27.860026 & 42.544976 \\
 & 3 & 131.439985 & 6.354504 & 72.531599 & \bfseries 1.912940 & 20.684538 & 1.812175 & 3.321852 & 37.916293 & 68.710977 \\
 & 4 & 291.343519 & 10.107835 & 132.586297 & \bfseries 3.701794 & 28.823535 & 2.197388 & 2.730523 & 35.816768 & 78.703331 \\
 & 5 & 609.770946 & 16.502311 & 232.846945 & \bfseries 7.591218 & 36.950640 & 2.618763 & 2.173869 & 30.673201 & 80.325841 \\
 & 6 & 1073.577423 & 30.583644 & 400.906176 & \bfseries 17.996505 & 35.102992 & 2.677877 & 1.699421 & 22.276891 & 59.654774 \\
 & 7 & 2475.523333 & 61.944951 & 686.155049 & \bfseries 44.783922 & 39.963279 & 3.607819 & 1.383196 & 15.321460 & 55.277055 \\
 & 8 & nan & 149.661328 & 1093.960800 & \bfseries 124.578619 & nan & nan & 1.201340 & 8.781289 & nan \\
 & 9 & nan & 399.637027 & 1964.354683 & \bfseries 359.406467 & nan & nan & 1.111936 & 5.465552 & nan \\
\bottomrule
\end{tabular}\end{adjustbox}
\end{table}

